In-Network Computing With Function as a Service at the Edge

Offloading computation from user devices to nodes with processing capabilities at the edge of the network is a major trend in today's network/service architectures. At the same time, serverless computing has gained a huge traction among the cloud computing technologies and has, thus, promoted the adoption of Function-as-a-Service (FaaS). The latter has some characteristics that make it generally suitable to edge applications, except for its cumbersome support of stateful applications. This work is set to provide a broad view on the options available for supporting stateful FaaS, which are distilled into four reference execution models that differ on where the state resides. While further investigation is needed to advance our understanding of the opportunities offered by in-network computing through stateful FaaS, initial insights are provided by means of a qualitative analysis of the four alternatives and their quantitative comparison in a simulator.

==> biographies.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/claudio}}]{Claudio Cicconetti}%
  \input{bios/claudio}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/marco}}]{Marco Conti}%
  \input{bios/marco}
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
% \newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/andrea}}]{Andrea Passarella}%
  \input{bios/andrea}
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.
% \vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
% \enlargethispage{-5in}

